Overview of KAGRA: Calibration, detector characterization, physical environmental monitors, and the geophysics interferometer

KAGRA is a newly built gravitational wave observatory, a laser interferometer with a 3 km arm length, located in Kamioka, Gifu, Japan. In this series of articles, we present an overview of the baseline KAGRA, for which we finished installing the designed configuration in 2019. This article describes the method of calibration (CAL) used for reconstructing gravitational wave signals from the detector outputs, as well as the characterization of the detector (DET). We also review the physical environmental monitors (PEM) system and the geophysics interferometer (GIF). Both are used for characterizing and evaluating the data quality of the gravitational wave channel. They play important roles in utilizing the detector output for gravitational wave searches. These characterization investigations will be even more important in the near future, once gravitational wave detection has been achieved, and in using KAGRA in the gravitational wave astronomy era.

==> ptep03_author.tex <==
\author[1,2]{T.~Akutsu}
\author[3,4,1]{M.~Ando}
\author[5]{K.~Arai}
\author[5]{Y.~Arai}
\author[6]{S.~Araki}
\author[7]{A.~Araya}
\author[3]{N.~Aritomi}
\author[8]{H.~Asada}
\author[9,10]{Y.~Aso}
\author[11]{S.~Bae}
\author[12]{Y.~Bae}
\author[13]{L.~Baiotti}
\author[14]{R.~Bajpai}
\author[1]{M.~A.~Barton}
\author[4]{K.~Cannon}
\author[15]{Z.~Cao}
\author[1]{E.~Capocasa}
\author[16]{M.~Chan}
\author[17,18]{C.~Chen}
\author[19]{K.~Chen}
\author[18]{Y.~Chen}
\author[20]{C-Y.~Chiang}
\author[19]{H.~Chu}
\author[20]{Y-K.~Chu}
\author[16]{S.~Eguchi}
\author[3]{Y.~Enomoto}
\author[21,1]{R.~Flaminio}
\author[22]{Y.~Fujii}
\author[23]{Y.~FUJIKAWA}
\author[5]{M.~Fukunaga}
\author[2]{M.~Fukushima}
\author[24]{D.~Gao}
\author[24]{G.~Ge}
\author[25]{S.~Ha}
\author[5,26]{A.~Hagiwara}
\author[20]{S.~Haino}
\author[27]{W.-B.~Han}
\author[5]{K.~Hasegawa}
\author[28]{K.~Hattori}
\author[29]{H.~Hayakawa}
\author[16]{K.~Hayama}
\author[30]{Y.~Himemoto}
\author[31]{Y.~Hiranuma}
\author[1]{N.~Hirata}
\author[5]{E.~Hirose}
\author[32]{Z.~Hong}
\author[5]{B.~Hsieh}
\author[32]{G-Z.~Huang}
\author[20]{H-Y.~Huang}
\author[24]{P.~Huang}
\author[18]{Y-C.~Huang}
\author[20]{Y.~Huang}
\author[33]{D.~C.~Y.~Hui}
\author[34]{S.~Ide}
\author[2]{B.~Ikenoue}
\author[32]{S.~Imam}
\author[35]{K.~Inayoshi}
\author[19]{Y.~Inoue}
\author[36]{K.~Ioka}
\author[37]{K.~Ito}
\author[38,39]{Y.~Itoh}
\author[40]{K.~Izumi}
\author[41]{C.~Jeon}
\author[42,43]{H.-B.~Jin}
\author[25]{K.~Jung}
\author[29]{P.~Jung}
\author[37]{K.~Kaihotsu}
\author[44]{T.~Kajita}
\author[45]{M.~Kakizaki}
\author[29]{M.~Kamiizumi}
\author[38,39]{N.~Kanda}
\author[11]{G.~Kang}
\author[5]{K.~Kawaguchi}
\author[46]{N.~Kawai}
\author[3]{T.~Kawasaki}
\author[41]{C.~Kim}
\author[47]{J.~Kim}
\author[48]{J.~C.~Kim}
\author[12]{W.~S.~Kim}
\author[25]{Y.-M.~Kim}
\author[26]{N.~Kimura}
\author[3]{N.~Kita}
\author[37]{H.~Kitazawa}
\author[49]{Y.~Kojima}
\author[29]{K.~Kokeyama}
\author[3]{K.~Komori}
\author[18]{A.~K.~H.~Kong}
\author[16]{K.~Kotake}
\author[9]{C.~Kozakai}
\author[50]{R.~Kozu}
\author[51]{R.~Kumar}
\author[4]{J.~Kume}
\author[19]{C.~Kuo}
\author[32]{H-S.~Kuo}
\author[37]{Y.~Kuromiya}
\author[52]{S.~Kuroyanagi}
\author[46]{K.~Kusayanagi}
\author[25]{K.~Kwak}
\author[53]{H.~K.~Lee}
\author[48]{H.~W.~Lee}
\author[18]{R.~Lee}
\author[1]{M.~Leonardi}
\author[18]{K.~L.~Li}
\author[25]{L.~C.-C.~Lin}
\author[54]{C-Y.~Lin}
\author[20]{F-K.~Lin}
\author[32]{F-L.~Lin}
\author[19]{H.~L.~Lin}
\author[17]{G.~C.~Liu}
\author[20]{L.-W.~Luo}
\author[55]{E.~Majorana}
\author[1]{M.~Marchio}
\author[3]{Y.~Michimura}
\author[56]{N.~Mio}
\author[29]{O.~Miyakawa}
\author[38]{A.~Miyamoto}
\author[3]{Y.~Miyazaki}
\author[29]{K.~Miyo}
\author[29]{S.~Miyoki}
\author[37]{Y.~Mori}
\author[5]{S.~Morisaki}
\author[45]{Y.~Moriwaki}
\author[40]{K.~Nagano}
\author[57]{S.~Nagano}
\author[1]{K.~Nakamura}
\author[58]{H.~Nakano}
\author[5]{M.~Nakano}
\author[46]{R.~Nakashima}
\author[28]{Y.~Nakayama}
\author[5]{T.~Narikawa}
\author[55]{L.~Naticchioni}
\author[31]{R.~Negishi}
\author[59]{L.~Nguyen Quynh}
\author[42,24,60]{W.-T.~Ni}
\author[4]{A.~Nishizawa}
\author[28]{S.~Nozaki}
\author[2]{Y.~Obuchi}
\author[5]{W.~Ogaki}
\author[12]{J.~J.~Oh}
\author[33]{K.~Oh}
\author[12]{S.~H.~Oh}
\author[29]{M.~Ohashi}
\author[9]{N.~Ohishi}
\author[23]{M.~Ohkawa}
\author[4]{H.~Ohta}
\author[34]{Y.~Okutani}
\author[29]{K.~Okutomi}
\author[31]{K.~Oohara}
\author[3]{C.~Ooi}
\author[29]{S.~Oshino}
\author[46]{S.~Otabe}
\author[18]{K.~Pan}
\author[19]{H.~Pang}
\author[17]{A.~Parisi}
\author[61]{J.~Park}
\author[29]{F.~E.~Pe\~na Arellano}
\author[62]{I.~Pinto}
\author[63]{N.~Sago}
\author[2]{S.~Saito}
\author[29]{Y.~Saito}
\author[64]{K.~Sakai}
\author[31]{Y.~Sakai}
\author[16]{Y.~Sakuno}
\author[65]{S.~Sato}
\author[23]{T.~Sato}
\author[38]{T.~Sawada}
\author[4]{T.~Sekiguchi}
\author[66]{Y.~Sekiguchi}
\author[35]{L.~Shao}
\author[16]{S.~Shibagaki}
\author[2]{R.~Shimizu}
\author[3]{T.~Shimoda}
\author[29]{K.~Shimode}
\author[67]{H.~Shinkai}
\author[10]{T.~Shishido}
\author[1]{A.~Shoda}
\author[46]{K.~Somiya}
\author[12]{E.~J.~Son}
\author[68]{H.~Sotani}
\author[69,40]{R.~Sugimoto}
\author[5]{J.~Suresh}
\author[23]{T.~Suzuki}
\author[5]{T.~Suzuki}
\author[5]{H.~Tagoshi}
\author[70]{H.~Takahashi}
\author[1]{R.~Takahashi}
\author[7]{A.~Takamori}
\author[3]{S.~Takano}
\author[3]{H.~Takeda}
\author[38]{M.~Takeda}
\author[71]{H.~Tanaka}
\author[38]{K.~Tanaka}
\author[71]{K.~Tanaka}
\author[5]{T.~Tanaka}
\author[63]{T.~Tanaka}
\author[1,10]{S.~Tanioka}
\author[1]{E.~N.~Tapia~San Martin}
\author[72]{S.~Telada}
\author[1]{T.~Tomaru}
\author[38]{Y.~Tomigami}
\author[29]{T.~Tomura}
\author[73,74]{F.~Travasso}
\author[29]{L.~Trozzo}
\author[75]{T.~Tsang}
\author[32]{J-S.~Tsao}
\author[3]{K.~Tsubono}
\author[38]{S.~Tsuchida}
\author[4]{T.~Tsutsui}
\author[2]{T.~Tsuzuki}
\author[20]{D.~Tuyenbayev}
\author[5]{N.~Uchikata}
\author[29]{T.~Uchiyama}
\author[26]{A.~Ueda}
\author[76,77]{T.~Uehara}
\author[4]{K.~Ueno}
\author[70]{G.~Ueshima}
\author[2]{F.~Uraguchi}
\author[5]{T.~Ushiba}
\author[78]{M.~H.~P.~M.~van ~Putten}
\author[74]{H.~Vocca}
\author[24]{J.~Wang}
\author[1]{T.~Washimi}
\author[18]{C.~Wu}
\author[18]{H.~Wu}
\author[18]{S.~Wu}
\author[32]{W-R.~Xu}
\author[71]{T.~Yamada}
\author[45]{K.~Yamamoto}
\author[71,81]{K.~Yamamoto}
\author[29]{T.~Yamamoto}
\author[28]{K.~Yamashita}
\author[34]{R.~Yamazaki}
\author[79]{Y.~Yang}
\author[37]{K.~Yokogawa}
\author[4,3]{J.~Yokoyama}
\author[29]{T.~Yokozawa}
\author[37]{T.~Yoshioka}
\author[5]{H.~Yuzurihara}
\author[80]{S.~Zeidler}
\author[24]{M.~Zhan}
\author[32]{H.~Zhang}
\author[1]{Y.~Zhao}
\author[15]{Z.-H.~Zhu}

\affil[1]{Gravitational Wave Science Project, National Astronomical Observatory of Japan (NAOJ), 2-21-1 Osawa, Mitaka City, Tokyo 181-8588, Japan}
\affil[2]{Advanced Technology Center, National Astronomical Observatory of Japan (NAOJ), 2-21-1 Osawa, Mitaka City, Tokyo 181-8588, Japan}
\affil[3]{Department of Physics, The University of Tokyo, 7-3-1 Hongo, Bunkyo-ku, Tokyo 113-0033, Japan}
\affil[4]{Research Center for the Early Universe (RESCEU), The University of Tokyo, 7-3-1 Hongo, Bunkyo-ku, Tokyo 113-0033, Japan}
\affil[5]{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, 5-1-5 Kashiwa-no-Ha, Kashiwa City, Chiba 277-8582, Japan}
\affil[6]{Accelerator Laboratory, High Energy Accelerator Research Organization (KEK), 1-1 Oho, Tsukuba City, Ibaraki 305-0801, Japan}
\affil[7]{Earthquake Research Institute, The University of Tokyo, 1-1-1 Yayoi, Bunkyo-ku, Tokyo 113-0032, Japan}
\affil[8]{Department of Mathematics and Physics, Hirosaki University, 3 Bunkyo-cho, Hirosaki City, Aomori 036-8561, Japan}
\affil[9]{Kamioka Branch, National Astronomical Observatory of Japan (NAOJ), 238 Higashi-Mozumi, Kamioka-cho, Hida City, Gifu 506-1205, Japan}
\affil[10]{The Graduate University for Advanced Studies (SOKENDAI), 2-21-1 Osawa, Mitaka City, Tokyo 181-8588, Japan}
\affil[11]{Korea Institute of Science and Technology Information (KISTI), 245 Daehak-ro, Yuseong-gu, Daejeon 34141, Korea}
\affil[12]{National Institute for Mathematical Sciences, 70 Yuseong-daero, 1689 Beon-gil, Yuseong-gu, Daejeon 34047, Korea}
\affil[13]{International College, Osaka University, 1-1 Machikaneyama-cho, Toyonaka City, Osaka 560-0043, Japan}
\affil[14]{School of High Energy Accelerator Science, The Graduate University for Advanced Studies (SOKENDAI), 1-1 Oho, Tsukuba City, Ibaraki 305-0801, Japan}
\affil[15]{Department of Astronomy, Beijing Normal University, No. 19 Xinjiekou Street, Beijing 100875, China}
\affil[16]{Department of Applied Physics, Fukuoka University, 8-19-1 Nanakuma, Jonan, Fukuoka City, Fukuoka 814-0180, Japan}
\affil[17]{Department of Physics, Tamkang University, No. 151, Yingzhuan Rd., Danshui Dist., New Taipei City 25137, Taiwan}
\affil[18]{Department of Physics and Institute of Astronomy, National Tsing Hua University, No. 101 Section 2, Kuang-Fu Road,  Hsinchu 30013, Taiwan}
\affil[19]{Department of Physics, Center for High Energy and High Field Physics, National Central University, No.300, Zhongda Rd, Zhongli District, Taoyuan City 32001, Taiwan}
\affil[20]{Institute of Physics, Academia Sinica, 128 Sec. 2, Academia Rd., Nankang, Taipei 11529, Taiwan}
\affil[21]{Univ. Grenoble Alpes, Laboratoire d'Annecy de Physique des Particules (LAPP),  Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France}
\affil[22]{Department of Astronomy, The University of Tokyo, 2-21-1 Osawa, Mitaka City, Tokyo 181-8588, Japan}
\affil[23]{Faculty of Engineering, Niigata University, 8050 Ikarashi-2-no-cho, Nishi-ku, Niigata City, Niigata 950-2181, Japan}
\affil[24]{State Key Laboratory of Magnetic Resonance and Atomic and Molecular Physics, Innovation Academy for Precision Measurement Science and Technology (APM), Chinese Academy of Sciences, West No. 30, Xiao Hong Shan, Wuhan 430071, China}
\affil[25]{Department of Physics, School of Natural Science, Ulsan National Institute of Science and Technology (UNIST), 50 UNIST-gil, Ulju-gun, Ulsan 44919, Korea}
\affil[26]{Applied Research Laboratory, High Energy Accelerator Research Organization (KEK), 1-1 Oho, Tsukuba City, Ibaraki 305-0801, Japan}
\affil[27]{Chinese Academy of Sciences, Shanghai Astronomical Observatory, 80 Nandan Road, Shanghai 200030, China}
\affil[28]{Faculty of Science, University of Toyama, 3190 Gofuku, Toyama City, Toyama 930-8555, Japan}
\affil[29]{Institute for Cosmic Ray Research (ICRR), KAGRA Observatory, The University of Tokyo, 238 Higashi-Mozumi, Kamioka-cho, Hida City, Gifu 506-1205, Japan}
\affil[30]{College of Industrial Technology, Nihon University, 1-2-1 Izumi, Narashino City, Chiba 275-8575, Japan}
\affil[31]{Graduate School of Science and Technology, Niigata University, 8050 Ikarashi-2-no-cho, Nishi-ku, Niigata City, Niigata 950-2181, Japan}
\affil[32]{Department of Physics, National Taiwan Normal University, 88 Ting-Chou Rd. , sec. 4, Taipei 116, Taiwan}
\affil[33]{Astronomy \& Space Science, Chungnam National University, 9 Daehak-ro,  Yuseong-gu, Daejeon 34134, Korea, Korea}
\affil[34]{Department of Physics and Mathematics, Aoyama Gakuin University, 5-10-1 Fuchinobe, Sagamihara City, Kanagawa  252-5258, Japan}
\affil[35]{Kavli Institute for Astronomy and Astrophysics, Peking University, Yiheyuan Road 5, Haidian District, Beijing 100871, China}
\affil[36]{Yukawa Institute for Theoretical Physics (YITP), Kyoto University, Kita-Shirakawa Oiwake-cho, Sakyou-ku, Kyoto City, Kyoto 606-8502, Japan}
\affil[37]{Graduate School of Science and Engineering, University of Toyama, 3190 Gofuku, Toyama City, Toyama 930-8555, Japan}
\affil[38]{Department of Physics, Graduate School of Science, Osaka City University, 3-3-138 Sugimoto-cho, Sumiyoshi-ku, Osaka City, Osaka 558-8585, Japan}
\affil[39]{Nambu Yoichiro Institute of Theoretical and Experimental Physics (NITEP), Osaka City University, 3-3-138 Sugimoto-cho, Sumiyoshi-ku, Osaka City, Osaka 558-8585, Japan}
\affil[40]{Institute of Space and Astronautical Science (JAXA), 3-1-1 Yoshinodai, Chuo-ku, Sagamihara City, Kanagawa 252-0222, Japan}
\affil[41]{Department of Physics, Ewha Womans University, 52 Ewhayeodae, Seodaemun-gu, Seoul 03760, Korea}
\affil[42]{National Astronomical Observatories, Chinese Academic of Sciences, 20A Datun Road, Chaoyang District, Beijing, China}
\affil[43]{School of Astronomy and Space Science, University of Chinese Academy of Sciences, 20A Datun Road, Chaoyang District, Beijing, China}
\affil[44]{Institute for Cosmic Ray Research (ICRR), The University of Tokyo, 5-1-5 Kashiwa-no-Ha, Kashiwa City, Chiba 277-8582, Japan}
\affil[45]{Faculty of Science, University of Toyama, 3190 Gofuku, Toyama City, Toyama 930-8555, Japan}
\affil[46]{Graduate School of Science and Technology, Tokyo Institute of Technology, 2-12-1 Ookayama, Meguro-ku, Tokyo 152-8551, Japan}
\affil[47]{Department of Physics, Myongji University,  Yongin 17058, Korea}
\affil[48]{Department of Computer Simulation, Inje University, 197 Inje-ro, Gimhae, Gyeongsangnam-do 50834, Korea}
\affil[49]{Department of Physical Science, Hiroshima University, 1-3-1 Kagamiyama, Higashihiroshima City, Hiroshima 903-0213, Japan}
\affil[50]{Institute for Cosmic Ray Research (ICRR), Research Center for Cosmic Neutrinos (RCCN), The University of Tokyo, 238 Higashi-Mozumi, Kamioka-cho, Hida City, Gifu 506-1205, Japan}
\affil[51]{California Institute of Technology, 1200 East California Boulevard, Pasadena, CA 91125, USA}
\affil[52]{Institute for Advanced Research, Nagoya University, ES bldg. 604, Furocho, Chikusa-ku, Nagoya City, Aichi 464-8602, Japan}
\affil[53]{Department of Physics, Hanyang University, Wangsimniro 222, Sungdong-gu, Seoul 04763, Korea}
\affil[54]{National Center for High-performance computing, National Applied Research Laboratories, No. 7, R\&D 6th Rd., Hsinchu Science Park, Hsinchu City 30076, Taiwan}
\affil[55]{Istituto Nazionale di Fisica Nucleare (INFN), Universita di Roma "La Sapienza", P.le A. Moro 2, 00185 Roma, Italy}
\affil[56]{Institute for Photon Science and Technology, The University of Tokyo, 2-11-16 Yayoi, Bunkyo-ku, Tokyo 113-8656, Japan}
\affil[57]{The Applied Electromagnetic Research Institute, National Institute of Information and Communications Technology (NICT), 4-2-1 Nukuikita-machi, Koganei City, Tokyo 184-8795, Japan}
\affil[58]{Faculty of Law, Ryukoku University, 67 Fukakusa Tsukamoto-cho, Fushimi-ku, Kyoto City, Kyoto 612-8577, Japan}
\affil[59]{Department of Physics, University of Notre Dame, 225 Nieuwland Science Hall, Notre Dame, IN 46556, USA}
\affil[60]{Department of Physics, National Tsing Hua University, No. 101 Section 2, Kuang-Fu Road,  Hsinchu 30013, Taiwan}
\affil[61]{Korea Astronomy and Space Science Institute (KASI), 776 Daedeokdae-ro, Yuseong-gu, Daejeon 34055, Korea}
\affil[62]{Department of Engineering, University of Sannio,  Benevento 82100, Italy}
\affil[63]{Department of Physics, Kyoto University, Kita-Shirakawa Oiwake-cho, Sakyou-ku, Kyoto City, Kyoto 606-8502, Japan}
\affil[64]{Department of Electronic Control Engineering, National Institute of Technology, Nagaoka College, 888 Nishikatakai, Nagaoka City, Niigata 940-8532, Japan}
\affil[65]{Graduate School of Science and Engineering, Hosei University, 3-7-2 Kajino, Koganei City, Tokyo 184-8584, Japan}
\affil[66]{Faculty of Science, Toho University, 2-2-1 Miyama, Funabashi City, Chiba 274-8510, Japan}
\affil[67]{Faculty of Information Science and Technology, Osaka Institute of Technology, 1-79-1 Kitayama, Hirakata City, Osaka 573-0196, Japan}
\affil[68]{iTHEMS (Interdisciplinary Theoretical and Mathematical Sciences Program), The Institute of Physical and Chemical Research (RIKEN), 2-1 Hirosawa, Wako, Saitama 351-0198, Japan}
\affil[69]{Department of Space and Astronautical Science, The Graduate University for Advanced Studies (SOKENDAI), 3-1-1 Yoshinodai, Chuo-ku,, Sagamihara, Kanagawa 252-5210, Japan}
\affil[70]{Department of Information and Management  Systems Engineering, Nagaoka University of Technology, 1603-1 Kamitomioka, Nagaoka City, Niigata 940-2188, Japan}
\affil[71]{Institute for Cosmic Ray Research (ICRR), Research Center for Cosmic Neutrinos (RCCN), The University of Tokyo, 5-1-5 Kashiwa-no-Ha, Kashiwa City, Chiba 277-8582, Japan}
\affil[72]{National Metrology Institute of Japan, National Institute of Advanced Industrial Science and Technology, 1-1-1 Umezono, Tsukuba City, Ibaraki 305-8568, Japan}
\affil[73]{University of Camerino, via Madonna delle Carderi 9, 62032 Camerino (MC), Italy}
\affil[74]{Istituto Nazionale di Fisica Nucleare, University of Perugia, Via Pascoli 1, Perugia 06123, Italy}
\affil[75]{Faculty of Science, Department of Physics, The Chinese University of Hong Kong,  Shatin, N.T., Hong Kong}
\affil[76]{Department of Communications Engineering, National Defense Academy of Japan, 1-10-20 Hashirimizu, Yokosuka City, Kanagawa 239-8686, Japan}
\affil[77]{Department of Physics, University of Florida,  Gainesville, FL 32611, USA}
\affil[78]{Department of Physics and Astronomy, Sejong University, 209 Neungdong-ro, Gwangjin-gu, Seoul 143-747, Korea}
\affil[79]{Department of Electrophysics, National Chiao Tung University, 101 Univ. Street, Hsinchu, Taiwan}
\affil[80]{Department of Physics, Rikkyo University, 3-34-1 Nishiikebukuro, Toshima-ku, Tokyo 171-8501, Japan}
\affil[81]{Max Planck Institute for Gravitational Physics (Albert Einstein Institute) and Institut für Gravitationsphysik, Leibniz Universität Hannover, Callinstrasse 38, 30167 Hannover, Germany}

